Understanding Regularized Spectral Clustering via Graph Conductance

This paper uses the relationship between graph conductance and spectral clustering to study (i) the failures of spectral clustering and (ii) the benefits of regularization. The explanation is simple. Sparse and stochastic graphs create a lot of small trees that are connected to the core of the graph by only one edge. Graph conductance is sensitive to these noisy `dangling sets'. Spectral clustering inherits this sensitivity. The second part of the paper starts from a previously proposed form of regularized spectral clustering and shows that it is related to the graph conductance on a `regularized graph'. We call the conductance on the regularized graph CoreCut. Based upon previous arguments that relate graph conductance to spectral clustering (e.g. Cheeger inequality), minimizing CoreCut relaxes to regularized spectral clustering. Simple inspection of CoreCut reveals why it is less sensitive to small cuts in the graph. Together, these results show that unbalanced partitions from spectral clustering can be understood as overfitting to noise in the periphery of a sparse and stochastic graph. Regularization fixes this overfitting. In addition to this statistical benefit, these results also demonstrate how regularization can improve the computational speed of spectral clustering. We provide simulations and data examples to illustrate these results.

==> KarlsSimulationSection.tex <==

These experiments aim to show three things.  First, that regularized spectral clustering finds a more balanced partition.  Second, vanilla spectral clustering is prone to ``catastrophic overfitting.’’  Third, computing the second eigenvector of $L_\tau$ takes less time than computing the second eigenvector of $L$.  This section studies 37 example networks from \url{http://snap.stanford.edu/data} \cite{snapnets}.  These networks were selected to be relatively easy to interpret and handle. The largest graph used is wiki-talk and has only 2,388,953 nodes in the largest component.  The complete list of graphs used is given below. There were no graphs that were initially selected, but later removed. Before computing anything, directed edges were symmetrized and nodes not connected to the largest connected component were removed.  Throughout all simulations, the regularization parameter $\tau$ is set to be the average degree of the graph.  This was not optimized, but is instead a previously proposed heuristic \cite{tai}. As defined in Section 2, the partitions are constructed by scanning through the second eigenvector.  Even though we argue that regularized approaches are trying to minimize \texttt{CoreCut}, every notion of conductance in this section is computed on the unregularized graph, including the scanning through the second eigenvector.  All eigen-computations were performed with \texttt{rARPACK} \cite{}.  

In this simulation, $1/2$ of the edges were removed from the graph and placed into a ``testing-set.’’  Refer to the remaining edges as the ``training-edges.’’ On the training-edges, the largest connected component was again identified.  Based upon that subset of the training-edges, the spectral partitions were formed.  


Each figure in this section corresponds to a different summary value (balance, training conductance, testing conductance, and running time).  In all figures, each point corresponds to a single network.  The $x$-axis corresponds to the summary value for regularized spectral clustering and the $y$-axis corresponds to the summary value for vanilla spectral clustering.  Each figure includes a black line, which is the line $x = y$.  All plots are on the log-log scale.  The size of each point corresponds to the number of nodes in the graph. 


In Figure \ref{fig:sim1}, the summary value is the number of nodes in the smaller partition set. Notice that the scales of the axes are entirely different.  Vanilla spectral clustering tends to identify sets with 100s of nodes or smaller.  However, regularizing tends increase the size of the sets into the 1000s.  


In Figure \ref{fig:sim2a}, the summary value is the conductance $\phi$ computed on the training-edges.  Because this is the quantity that Vanilla spectral clustering approximates, it is not surprising that it finds partitions with a smaller conductance.  However, Figure \ref{fig:2b} shows that if the conductance is computed using only edges in the testing-set, then sometimes the Vanilla sets have no internal edges (conductance =1).  We refer to this as catastrophic overfitting.  


In these simulations (and others), we found that the partitions produced by both forms of regularization \cite{amini2013pseudo} and \cite{chaudhuri2012spectral} are exactly equivalent.  We find it easier to implement fast code for \cite{chaudhuri2012spectral} and moreover, our implementations of it run faster.  Implementing \cite{amini2013pseudo} to take advantage of the sparsity in the graph requires defining a function which quickly multiplies a vector $x$ by $L_\tau$.  This can be done via $L_\tau x = x - D_\tau^{-1/2}AD_\tau^{-1/2}x - \tau/N \textbf{1}(\textbf{1} x)$.  However, with a user defined matrix multiplication, the eigensolver in \texttt{rARPACK} runs slightly slower. Because the regularized form from \cite{chaudhuri2012spectral} simply defines $L_\tau = I - D_\tau^{-1/2}AD_\tau^{-1/2}$, it can use the same eigensolver as Vanilla spectral clustering and, as such, the running times are more comparable.  Figure \ref{fig:sim3} uses this definition of regularized spectral clustering. Running times are from \texttt{rARPACK} computing two eigenvectors of $D_\tau^{-1/2}AD_\tau^{-1/2}$ and $D^{-1/2}AD^{-1/2}$ using the default settings.  A line of regression is added to Figure \ref{fig:sim3}.  The slope of this line is roughly 1.01 and its intercept is roughly .83.  


The list of SNAP networks is given here:amazon0302, amazon0312, amazon0505, amazon0601, ca-AstroPh, ca-CondMat, ca-GrQc, ca-HepPh, ca-HepTh, cit-HepPh, cit-HepTh, com-amazon.ungraph, com-youtube.ungraph, email-EuAll, email-Eu-core, facebook_combined, p2p-Gnutella04, p2p-Gnutella05, p2p-Gnutella06, p2p-Gnutella08, p2p-Gnutella09, p2p-Gnutella24, p2p-Gnutella25, p2p-Gnutella30, p2p-Gnutella31, roadNet-CA, roadNet-PA, roadNet-TX, soc-Epinions1, soc-Slashdot0811, soc-Slashdot0902, twitter_combined, web-Google, web-NotreDame, web-Stanford, wiki-Talk, wiki-Vote.

==> simulations_subsection.tex <==
In this section, we compare \texttt{Vanilla-SC} and \texttt{Regularized-SC} by simulations (Section \ref{sec:sim}) and real data examples (Section \ref{sec:real}).  

\subsection{Simulation}\label{sec:sim}

We simulate a random network with core and peripheries under Degree Corrected-Stochastic Blockmodel \cite{karrer2011stochastic}.  We simulate the core with 10000 nodes, four equal size blocks, average degree 100, and stochastic block matrix proportional to $\left(\begin{matrix}
0.8 & 0.2\\
0.2 & 0.8
\end{matrix}\right)$.  We simulate the periphery with 100 nodes and average degree 3, and the connections across core and periphery with average degree 0.002.  We set the regularizer $\tau$ to be average degree of the network.

%XXXXX FIGURE HERE XXXX
\begin{figure}[H]\centering 
	\vspace{-5pt}
	\subfigure{\label{fig:sim_vanilla}
		\includegraphics[width=0.3\columnwidth]{fig_eigen_Simulated_vanilla.pdf}
	}
	\subfigure{\label{fig:sim_reg}
		\includegraphics[width=0.3\columnwidth]{fig_eigen_Simulated_regularized.pdf}
	}
	\subfigure{\label{fig:sim_eigenval}
	\includegraphics[width=0.3\columnwidth]{fig_eigen_Simulated_regularized_eigenval.pdf}
}
\vspace{-5pt}
	\caption{The leading eigenvectors and eigenvalues of the simulated network. }
	\label{fig:sim}
	\vspace{-5pt}
\end{figure}

Figure \ref{fig:sim} shows the leading eigenvectors and eigenvalues for \texttt{Vanilla-SC} and \texttt{Regularized-SC}.  Without regularization, the leading eigenvectors localize on very few nodes, which leads \texttt{Vanilla-SC} to return very unbalanced partitions.   We show in Supplementary that even if we look through the 25 leading eigenvectors for \texttt{Vanilla-SC}, they are all highly localized, which means that \texttt{Vanilla-SC} fails to identify the four blocks. But by regularization, the four leading eigenvectors clearly reveals the block structure of the core.  The eigengap (between the 4th and 5th eigenvalue) also gets larger after regularization, which improves the computational efficiency, which we will discuss by real data examples in the following Section \ref{sec:real}.


